Resource Management in Fog/Edge Computing: A Survey

Contrary to using distant and centralized cloud data center resources, employing decentralized resources at the edge of a network for processing data closer to user devices, such as smartphones and tablets, is an upcoming computing paradigm, referred to as fog/edge computing. Fog/edge resources are typically resource-constrained, heterogeneous, and dynamic compared to the cloud, thereby making resource management an important challenge that needs to be addressed. This article reviews publications as early as 1991, with 85% of the publications between 2013-2018, to identify and classify the architectures, infrastructure, and underlying algorithms for managing resources in fog/edge computing.

==> sections/histogram-architecture.tex <==
2000 - 
2001 - 
2002 - 1
2003 - 1 
2004 - 1
2005 - 1
2006 - 11
2007 - 11
2008 - 
2009 - 
2010 - 
2011 - 11
2012 - 1
2013 - 1111111111
2014 - 111111111
2015 - 11111111111
2016 - 1111111111111
2017 - 1111111111111111111111
2018 - 111





==> sections/histogram-infrastructure.tex <==
2000 - 
2001 - 
2002 - 
2003 - 
2004 - 
2005 - 
2006 - 
2007 - 
2008 - 
2009 - 
2010 - 
2011 - 
2012 - 
2013 - 
2014 - 
2015 - 
2016 - 
2017 - 
2018 - 

